SliceNDice: Mining Suspicious Multi-attribute Entity Groups with Multi-view Graphs

Given the reach of web platforms, bad actors have considerable incentives to manipulate and defraud users at the expense of platform integrity. This has spurred research in numerous suspicious behavior detection tasks, including detection of sybil accounts, false information, and payment scams/fraud. In this paper, we draw the insight that many such initiatives can be tackled in a common framework by posing a detection task which seeks to find groups of entities which share too many properties with one another across multiple attributes (sybil accounts created at the same time and location, propaganda spreaders broadcasting articles with the same rhetoric and with similar reshares, etc.) Our work makes four core contributions: Firstly, we posit a novel formulation of this task as a multi-view graph mining problem, in which distinct views reflect distinct attribute similarities across entities, and contextual similarity and attribute importance are respected. Secondly, we propose a novel suspiciousness metric for scoring entity groups given the abnormality of their synchronicity across multiple views, which obeys intuitive desiderata that existing metrics do not. Finally, we propose the SliceNDice algorithm which enables efficient extraction of highly suspicious entity groups, and demonstrate its practicality in production, in terms of strong detection performance and discoveries on Snapchat's large advertiser ecosystem (89% precision and numerous discoveries of real fraud rings), marked outperformance of baselines (over 97% precision/recall in simulated settings) and linear scalability.

==> 090math.tex <==


\section{Setting Up Metric}

For any $N_ixN_i$ view $i$, each cell ${c_i \sim exp(\lambda_i)}$. There are $N_i^2$ cells, and so to estimate $\lambda_i$ we can use the MLE $\lambda_i = \frac{N_i^2}{M_i}$ where $N_i$ is the number of organizations and $M_i$ is the observed mass of all the cells in the view.


Convolving all the $N^2$ independent exponential distributions, we find that the total mass of the view $M_i \sim Gamma(N_i^2, \frac{N_i^2}{M_i})$. We assume that all the cells in the view follow the same distribution, and that the total mass of a block in the view $m_i \sim Gamma(n_i^2, \frac{N_i^2}{M_i}) $ where $n_i$ is the number of organizations in the block.  

Our suspiciousness metric for a single view is $-ln(p(m_i))$ where $p(x)$ is the value of the PDF of the block's mass and $m_i$ is the observed mass of the block. We use the following notation heretofor for the properties of view $i$: $m$ (observed mass of block), $M$ (observed mass of view), $n$ (\# of organizations in block), $N$ (\# of organizations in the view), $p^{-1}=$ ($\frac{n^2}{m}$),and  $P^{-1}=$ ($\frac{N^2}{M}$). 

The PDF of $Gamma(\alpha,\beta) =  \frac{\beta^\alpha}{\Gamma(\alpha)} x^{\alpha - 1} e^{-\beta x } $. Our suspiciousness function is therefore \\\\ $S = -ln(\frac{\beta^\alpha}{\Gamma(\alpha)} x^{\alpha - 1} e^{-\beta x }) = -ln(\frac{{P^{-1}}^{n^2}}{\Gamma(n^2)} m^{n^2 - 1} e^{-P^{-1} m }) = -ln(\frac{{P^{-1}}^{n^2}}{\Gamma(n^2)}) - ln(m^{n^2 - 1}) - ln(e^{-P^{-1} m })$


\section{Density Axiom}
Our axiom is that as the view's mass increases, and everything else is held constant, suspiciousness increases. Therefore we need to prove that $\frac{dS}{dm} > 0$ where $p > P$ (the density of the block is greater than the density of view). 

$\frac{dS}{dm} = \\   \frac{dS}{dm} (-ln(\frac{{P^{-1}}^{n^2}}{\Gamma(n^2)})) + \frac{dS}{dm}(-ln(m^{n^2 - 1})) + \frac{dS}{dm}(-ln(e^{-P^{-1} m })) =  \\ \frac{dS}{dm}(-ln(m^{n^2 - 1})) + \frac{dS}{dm}(-ln(e^{-P^{-1} m })) = \\ \frac{dS}{dm}(-(n^2 - 1)ln(m)) + \frac{dS}{dm}(P^{-1} m ) = \\
P^{-1}-\frac{n^2-1}{m} = \frac{N^2}{M}-\frac{n^2-1}{m}
$

Because $P < p$, $P^{-1} > p^{-1}$ which implies that $\frac{N^2}{M} > \frac{n^2}{m} > \frac{n^2-1}{m} $.

Therefore, $\frac{N^2}{M}-\frac{n^2-1}{m} > 0$ and so the suspiciousness only grows as the mass increases. 

\section{Size Axiom}

Our suspiciousness function (parameterized by density) is therefore

 $S = -ln(\frac{{P^{-1{n^2}}}}{\Gamma(n^2)}) - ln(m^{n^2 - 1}) - ln(e^{-P^{-1} m }) = \\ -ln(\frac{P^{-1{n^2}}}{\Gamma(n^2)}) - ln(m^{n^2 - 1}) + P^{-1} m = \\ -ln({P^{-1{n^2}}}) + ln(\Gamma(n^2)) - ln(m^{n^2 - 1}) + P^{-1} m = \\
 n^2ln(P) + ln(n^2!) - ln(n^2)  - (n^2 - 1)ln(m) + P^{-1} m = \\
 n^2ln(P) + ln(n^2!) - ln(n^2)  - n^2ln(m) + ln(m) + P^{-1} m= \\
 n^2ln(P) + n^2ln(n^2) - n^2 - ln(n^2)  - n^2ln(m) + ln(m) + P^{-1} m= \\
  n^2ln(P) + n^2ln(n^2) - n^2 - n^2ln(m) + ln(p) + P^{-1} m = \\
 n^2ln(P) - n^2ln(p) - n^2 + ln(p) + P^{-1} m = \\
  n^2ln(P) - n^2ln(p) - n^2 + ln(p) + \frac{n^2p}{P}$
  
We now the derivative of each of the above.

$\frac{dS}{dn} =  2n*ln(P) - 2nln(p) - 2n + 2n(p/P) = \\ 
2n(ln(P) - ln(p) + p/P - 1 ) = \\
2n(ln(P/p) + p/P - 1 ) = \\ 
2n(p/P - ln(p/P) - 1 )$

Because $x-log(x) > 1$ when $x > 1$, the above equation is always positive given that we are assuming that $p > P$.

\section{Concentration Axiom}

We start with the derivative  of the suspiciousness metric derived above:

$\frac{d}{dn}(n^2ln(P) + n^2ln(n^2) - n^2 - ln(n^2)  - n^2ln(m) + ln(m) + P^{-1} m) = \\
2n*ln(P) + 2n(ln(n^2)+1) - 2n - \frac{2}{n} - 2n*ln(m) = \\
2n(ln(P) + ln(n^2) + 1 - 1 - \frac{1}{n^2} - ln(m)) = \\
2n(ln(P) + ln(p^{-1}) - \frac{1}{n^2}) = 
2n(ln(P/p) - \frac{1}{n^2}) = \\
2n(-ln(p/P) - \frac{1}{n^2} )$

We know that $-ln(p/P) <= -1$ because $p/P > 1$, so therefore the sign of the above is negative. This implies that suspiciousness of a block grows as volume decreases, assuming mass is held constant. 

\section{Contrast Axiom}

$\frac{dS}{dP}(n^2ln(P) - n^2ln(p) - n^2 + ln(p) + \frac{n^2p}{P}) = \\
\frac{dS}{dP}(n^2ln(P) + n^2pP^{-1}) = \\
n^2P^{-1} - n^2pP^{-2} = \\
n^2(P^{-1} - P^{-1}\frac{p}{P}) < 0$


 
\section{Relationship to KL Divergence}

We start with the simplified form of the log-likihood version of the suspiciousness metric:

Our suspiciousness function is therefore

 $S = -ln(\frac{{P^{-1{n^2}}}}{\Gamma(n^2)}) - ln(m^{n^2 - 1}) - ln(e^{-P^{-1} m }) = \\ -ln(\frac{P^{-1{n^2}}}{\Gamma(n^2)}) - ln(m^{n^2 - 1}) + P^{-1} m = \\ -ln({P^{-1{n^2}}}) + ln(\Gamma(n^2)) - ln(m^{n^2 - 1}) + P^{-1} m$



Now, we look at the product of the number of cells in the block and the KL divergences of a single cell's value in the block and the view:

$n^2 D_{KL}(exp(p^{-1}),exp(P^{-1})) = \\ n^2(ln(p^{-1}) - ln(P^{-1}) + \frac{P^{-1}}{p^{-1}} - 1) = \\ 
n^2ln(p^{-1}) - n^2ln(P^{-1}) + n^2\frac{P^{-1}}{p^{-1}} - n^2 = \\
n^2ln(p^{-1}) - n^2ln(P^{-1}) + n^2\frac{P^{-1}}{\frac{n^2}{m}} - n^2 = \\
n^2ln(p^{-1}) - ln(P^{-1{n^2}}) + P^{-1}m - n^2 =$


The 1st/4th term from the suspiciousness function and the 2nd/3rd terms from the KL divergence are the same. Removing these, we are left with.

$S =  ln(\Gamma(n^2)) - ln(m^{n^2 - 1}) = \\ 
(n^2-1)ln(n^2-1) - (n^2 -1) - (n^2-1)ln(m) = \\
(n^2-1)(ln(n^2-1) - ln(m) -1) = \\
(n^2-1) (ln(\frac{n^2-1}{m})-1)$

and

$KL = n^2ln(p^{-1}) - n^2 = \\
n^2(ln(p^{-1}) -1) = \\
n^2(ln(n^2/m)-1)$
